Planning as Inference in Epidemiological Models

In this work we demonstrate how to automate parts of the infectious disease-control policy-making process via performing inference in existing epidemiological models. The kind of inference tasks undertaken include computing the posterior distribution over controllable, via direct policy-making choices, simulation model parameters that give rise to acceptable disease progression outcomes. Among other things, we illustrate the use of a probabilistic programming language that automates inference in existing simulators. Neither the full capabilities of this tool for automating inference nor its utility for planning is widely disseminated at the current time. Timely gains in understanding about how such simulation-based models and inference automation tools applied in support of policymaking could lead to less economically damaging policy prescriptions, particularly during the current COVID-19 pandemic.

==> figures/FRED_tex/_fig_scatter_vancouver.tex <==
\begin{figure}
    \centering

    \begin{subfigure}[b]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/FRED/revised/kde_vancouver-past_success.pdf}
        \caption{Before June 2021.}
        \label{fig:FRED-scatter-plot-grid:before}
    \end{subfigure}

    \begin{subfigure}[b]{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/FRED/revised/kde_vancouver-future_success.pdf}
        \caption{After June 2021.}
        \label{fig:FRED-scatter-plot-grid:after}
    \end{subfigure}

    \caption{Empirically determined marginals of the full joint distribution over controllable policy parameters showing the probability that each parameter value leads to appropriately controlled outcomes (see Equation \eqref{eq:control-inference}) for simulations of COVID-19 in Vancouver.  The bottom row of each figure shows one-dimensional marginals for each policy parameter, with the the uniform prior indicated by the dashed line.  Figure \ref{fig:FRED-scatter-plot-grid:before} shows result for simulations for the six months before June 2021, whereas Figure \ref{fig:FRED-scatter-plot-grid:after} shows results for simulations for the six months after June 2021.  The remaining array of plots show kernel density estimate (KDE) plots (using Gaussian kernels) for the two-dimensional marginals of the joint distribution.  Darker green indicates higher density.  \aw{CHECK THIS: We see that in the six months priors to June 2021, when cases are high, school closures and social distancing are very effective policy measures.  After June 2021, when case rates are lower, a broader range of controls are available to achieve the desired objective.  This richly structured, policy-level information is only available through the application of Bayesian analysis, such that the resulting distributions are ``well-calibrated'' \sn{I'm against including the ``well-calibrated'' word. We don't have a proper definition of it.} and can be compared in this manner.}}
    \label{fig:FRED-scatter-plot-grid-vancouver}
\end{figure}


==> figures/FRED_tex/_fig_summaries_vancouver.tex <==
\begin{figure}
    \centering
    % \includegraphics[width=0.49\textwidth]{figures/FRED/allegheny_controlled.pdf}
    % \includegraphics[width=0.49\textwidth]{figures/FRED/allegheny_uncontrolled.pdf}
    
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/FRED/vancouver/h1/cases.pdf}
        
        \includegraphics[width=\textwidth]{figures/FRED/vancouver/h1/hospitalizations.pdf}
        
        \includegraphics[width=\textwidth]{figures/FRED/vancouver/h1/deaths.pdf}
        \caption{Before June 2021.}
        \label{fig:timeseries-vancouver-past}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/FRED/vancouver/h2/cases.pdf}
        
        \includegraphics[width=\textwidth]{figures/FRED/vancouver/h2/hospitalizations.pdf}
        
        \includegraphics[width=\textwidth]{figures/FRED/vancouver/h2/deaths.pdf}
        \caption{After June 2021s.}
        \label{fig:timeseries-vancouver}
    \end{subfigure}
    \caption{}
    \label{fig:timeseries-vancouver-future}
\end{figure} 

% \begin{figure}
%     \centering
%     \includegraphics{figures/FRED/vancouver/h1/cases.pdf}
%     \caption{Cases in Vancouver in the first half of 2021.}
%     \label{fig:vancouver_cases1}
% \end{figure}
%
% \begin{figure}
%     \centering
%     \includegraphics{figures/FRED/vancouver/h1/hospitalizations.pdf}
%     \caption{Hospitalizations in Vancouver in the first half of 2021.}
%     \label{fig:vancouver_hospitalizations1}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics{figures/FRED/vancouver/h1/deaths.pdf}
%     \caption{Deaths in Vancouver in the first half of 2021.}
%     \label{fig:vancouver_deaths1}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics{figures/FRED/vancouver/h2/cases.pdf}
%     \caption{Cases in Vancouver in the second half of 2021.}
%     \label{fig:vancouver_cases2}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics{figures/FRED/vancouver/h2/hospitalizations.pdf}
%     \caption{Hospitalizations in Vancouver in the second half of 2021.}
%     \label{fig:vancouver_hospitalizations2}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics{figures/FRED/vancouver/h2/deaths.pdf}
%     \caption{Deaths in Vancouver in the second half of 2021.}
%     \label{fig:vancouver_deaths2}
% \end{figure}

==> figures/SEIR_tex/deterministic_controlled.tex <==
% moved to 06_models_1_seir.tex

==> figures/SEIR_tex/deterministic_simulation.tex <==
% moved to 06_models_1_seir.tex
